Do Time Constraints Re-Prioritize Attention to Shapes During Visual Photo Inspection?

People's visual experiences of the world are easy to carve up and examine along natural language boundaries, e.g., by category labels, attribute labels, etc. However, it is more difficult to elicit detailed visuospatial information about what a person attends to, e.g., the specific shape of a tree. Paying attention to the shapes of things not only feeds into well defined tasks like visual category learning, but it is also what enables us to differentiate similarly named objects and to take on creative visual pursuits, like poetically describing the shape of a thing, or finding shapes in the clouds or stars. We use a new data collection method that elicits people's prioritized attention to shapes during visual photo inspection by asking them to trace important parts of the image under varying time constraints. Using data collected via crowdsourcing over a set of 187 photographs, we examine changes in patterns of visual attention across individuals, across image types, and across time constraints.

==> scratchwork.tex <==
\begin{abstract}
People's visual experiences of the world are easy to carve up and examine along natural language boundaries, e.g., by category labels, attribute labels, etc.  However, it is more difficult to elicit detailed visuospatial information about what a person attends to, e.g., the specific shape of a tree.  Paying attention to the shapes of things not only feeds into well defined tasks like visual category learning, but it is also what enables us to differentiate similarly named objects and to take on creative visual pursuits, like poetically describing the shape of a thing, or finding shapes in the clouds or stars.  We use a new data collection method that elicits people's prioritized attention to shapes during visual photo inspection by asking them to trace important parts of the image under varying time constraints.  Using data collected via crowdsourcing over a set of 187 photographs, 
%Before an object is recognized, people pay attention to the shapes and sub-components that constitute it. It is natural to believe whatever shape people pay attention to first is the single most important sub-component of the object. However, shape can be hard to define, and recent studies have shown that many contour-based factors both directly and indirectly elicit attention. 
we examine changes in patterns of visual attention across individuals, across image types, and across time constraints.
%aim to determine if visual attention is drawn to shapes in a given image in the same order every time and if such behaviors would change under the influence of time pressure. Using line strokes from sketches as proxies for measuring attention on shapes, we asked participants to hand-trace a wide variety of photo images, spanning animals and geological formations, under different time constraints. 
We first mapped the sketches into 3D space, and then applied a heuristic for comparing sketch set similarity. By leveraging this technique on our collected dataset, we found that behaviors of visual production become more varied under time constraints and thus concluded that attention to shape-based properties is re-prioritized.

\textbf{Keywords:} 
crowdsourcing; edge detection; sketching; tracing; visual object perception.
\end{abstract}


\begin{table}[!ht]
\begin{center} 
\caption{Per Category Source Images} 
\setlength\tabcolsep{2pt}
\begin{tabular}{c c} 
\hline
Category &  Source Image Count \\
\hline
Abstract Shape & 20 \\
Animal & 20 \\
Artifacts & 42 \\
Faces & 20 \\
Food & 20 \\
Geological Formation & 20 \\
Natural Objects & 5 \\
People & 20 \\
Plant & 20 \\
\hline
\end{tabular} 
\end{center} 
\end{table}
